Adaptive parameters identification for nonlinear dynamics using deep permutation invariant networks

The promising outcomes of dynamical system identification techniques, such as SINDy [Brunton et al. 2016], highlight their advantages in providing qualitative interpretability and extrapolation compared to non-interpretable deep neural networks [Rudin 2019]. These techniques suffer from parameter updating in real-time use cases, especially when the system parameters are likely to change during or between processes. Recently, the OASIS [Bhadriraju et al. 2020] framework introduced a data-driven technique to address the limitations of real-time dynamical system parameters updating, yielding interesting results. Nevertheless, we show in this work that superior performance can be achieved using more advanced model architectures. We present an innovative encoding approach, based mainly on the use of Set Encoding methods of sequence data, which give accurate adaptive model identification for complex dynamic systems, with variable input time series length. Two Set Encoding methods are used, the first is Deep Set [Zaheer et al. 2017], and the second is Set Transformer [Lee et al. 2019]. Comparing Set Transformer to OASIS framework on Lotka Volterra for real-time local dynamical system identification and time series forecasting, we find that the Set Transformer architecture is well adapted to learning relationships within data sets. We then compare the two Set Encoding methods based on the Lorenz system for online global dynamical system identification. Finally, we trained a Deep Set model to perform identification and characterization of abnormalities for 1D heat-transfer problem.

==> tables/Tab.1.tex <==
\begin{table}[h]
\caption{Abbreviation table }\label{tab:abb_table}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Abbreviation}  & \textbf{Definition} \\
\midrule
CAE & Computer-Aided Engineering\\\hline
DMD & Dynamic Mode Decomposition \\\hline
DMDc & Dynamic Mode Decomposition with control \\\hline
DNN & Deep Neural Network \\\hline
EQL & EQuation Learning \\\hline
ISAB & Induced Self-Attention Block \\\hline
LASSO & Least Absolute Shrinkage and Selection Operator \\\hline
MAB & Multi-head Attention Block \\\hline
MAPE & Mean Absolute Percentage Error \\\hline
MLP & MultiLayer Perceptron \\\hline
MPC & Model Predictive Control \\\hline
NSODE & Neural Symbolic Ordinary Differential Equation \\\hline
OASIS & Operable Adaptive Sparse Identification of Systems \\\hline
OASIS-P & Online Adaptive Sparse Identification of Systems for Fault Prognosis \\\hline
ODE & Ordinary Differential Equation \\\hline
PINN & Physics Informed Neural Network \\\hline
PINN-SR & Physics Informed Neural Network with Sparse Regression \\\hline
PDE & Partial Differential Equation \\\hline
PMA & Pooling by Multihead Attention \\\hline
PySR & Python Symbolic Regression \\\hline
SAB & Self-Attention Block \\\hline
SENDI & Set Encoding for Nonlinear Dynamics Identification \\\hline
SGA-PDE & Symbolic Genetic Algorithm for discovering open-form Partial Differential Equations \\\hline
SINDYc & Sparse Identification of Nonlinear Dynamics with Control \\\hline
SINDy & Sparse Identification of Nonlinear Dynamics \\\hline
SR3 & Sparse Relaxed Regularized Regression \\\hline
rFF & row-wise FeedForward \\\hline
sMAPE & symmetric Mean Absolute Percentage Error \\
\botrule
\end{tabular}
\end{table}

==> tables/Tab.10.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set-Transformer and OASIS in terms of sMAPE error for extrapolation through local dynamics identification with a time window of 10 steps}
\label{RESL_10_smape}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{10}$ & $x$ & \textbf{0.47} & 1.23 & \textbf{1.11} & 3.58 & \textbf{5.36} & 44.64 \\
 & $y$ & \textbf{1.46} & 3.61 & \textbf{1.23} & 6.06 & \textbf{5.36} & 44.64 \\\midrule
2$\times \Delta t_{10}$ & $x$ & \textbf{1.96} & 3.40 & \textbf{6.07} & 12.20 & \textbf{5.36} & 42.86 \\
 & $y$ & \textbf{4.45} & 6.44 & \textbf{18.69} & 19.46 & \textbf{5.36} & 42.86 \\\midrule
3$\times \Delta t_{10}$ & $x$ & \textbf{2.31} & 4.23 & \textbf{5.78} & 13.59 & \textbf{7.14} & 41.07 \\
 & $y$ & \textbf{4.16} & 6.23 & \textbf{14.40} & 18.15 & \textbf{7.14} & 41.07 \\\midrule
4$\times \Delta t_{10}$ & $x$ & \textbf{4.51} & 5.87 & \textbf{13.44} & 16.14 & \textbf{3.57} & 39.29 \\
 & $y$ & \textbf{6.85} & 9.07 & 24.34 & \textbf{21.02} & \textbf{3.57} & 39.29 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.11.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set-Transformer and OASIS in terms of sMAPE error for extrapolation through local dynamics identification with a time window of 15 steps}
\label{RESL_15_smape}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{15}$ & $x$ & \textbf{1.14} & 1.76 & \textbf{1.87} & 3.01 & \textbf{7.14} & 51.79 \\
 & $y$ & \textbf{1.84} & 4.62 & \textbf{1.81} & 8.41 & \textbf{7.14} & 51.79 \\\midrule
2$\times \Delta t_{15}$ & $x$ & \textbf{2.69} & 3.78 & \textbf{5.07} & 10.55 & \textbf{7.14} & 51.79 \\
 & $y$ & \textbf{3.37} & 5.76 & \textbf{7.32} & 12.71 & \textbf{7.14} & 51.79 \\\midrule
3$\times \Delta t_{15}$ & $x$ & \textbf{4.60} & 6.13 & \textbf{6.03} & 13.73 & \textbf{5.36} & 44.64 \\
 & $y$ & \textbf{3.71} & 8.48 & \textbf{9.53} & 20.58 & \textbf{5.36} & 44.64 \\\midrule
4$\times \Delta t_{15}$ & $x$ & \textbf{7.40} & 9.56 & \textbf{14.88} & 24.25 & \textbf{3.57} & 44.64 \\
 & $y$ & \textbf{7.05} & 10.83 & \textbf{18.18} & 31.84 & \textbf{3.57} & 44.64 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.12.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set-Transformer and OASIS in terms of sMAPE error for extrapolation through local dynamics identification with a time window of 20 steps}
\label{RESL_20_smape}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{20}$ & $x$ & \textbf{2.63} & 2.66 & 3.92 & \textbf{2.24} & \textbf{7.14} & 55.36 \\
 & $y$ & \textbf{2.79} & 5.81 & \textbf{2.05} & 7.52 & \textbf{7.14} & 55.36 \\\midrule
2$\times \Delta t_{20}$ & $x$ & \textbf{6.21} & 7.35 & \textbf{11.32} & 24.77 & \textbf{7.14} & 50.00 \\
 & $y$ & \textbf{4.77} & 9.57 & \textbf{9.95} & 21.72 & \textbf{7.14} & 50.00 \\\midrule
3$\times \Delta t_{20}$ & $x$ & \textbf{9.82} & 11.83 & \textbf{23.89} & 25.61 & \textbf{7.14} & 44.64 \\
 & $y$ & \textbf{7.08} & 12.76 & \textbf{18.22} & 33.02 & \textbf{7.14} & 44.64 \\\midrule
4$\times \Delta t_{20}$ & $x$ & \textbf{9.88} & 12.51 & \textbf{16.45} & 35.09 & \textbf{3.57} & 53.57 \\
 & $y$ & \textbf{4.92} & 9.72 & \textbf{12.82} & 23.82 & \textbf{3.57} & 53.57 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.13.tex <==
\begin{table}[!htbp]
\centering\caption{Selected architecture for Deep Set method for all noise levels and all the parameters of the Lorenz system}
\label{tab:optimal_dpst}
\begin{tabular}{@{}llllc@{}}
\toprule
 & activation & Layers & Pooling                       & {\color[HTML]{0D0D0D} Trainable  parameter count} \\ \midrule
Encode & ReLU       & 320$\times5$  &                               &                                                   \\ 
Decode & ReLU       & 320$\times5$  & \multirow{-2}{*}{abs,   mean} & \multirow{-2}{*}{927043}                          \\ \botrule
\end{tabular}
\end{table}

==> tables/Tab.14.tex <==
\begin{table}[!htbp]
\centering\caption{Selected architecture for Set Transformer method for all noise levels and all the parameters of the Lorenz system}
\label{tab:optimal_trfs}
\begin{tabular}{@{}lllc@{}}
\hline
 & Attention   blocks & rFF & {\color[HTML]{0D0D0D} Trainable   parameter count} \\ \hline
Encode & ISAB($d=45,   m=128, h=40$) & rFF(45, 2, ReLU) &  \\ 
Pooling & PAM($k=1, d=40, h=40$) & rFF(40, 2, ReLU) & \multirow{-2}{*}{1045733}  \\ \botrule
\end{tabular}
\end{table}

==> tables/Tab.15.tex <==
\begin{table}[!htbp]
\centering
\caption{Selected architecture for the Deep Set method for all noise levels in the third application}
\label{tab:optimal_dpst_app3}
\begin{tabular}{@{}llllc@{}}
\toprule
 & Activation & Layers & Pooling & {\color[HTML]{0D0D0D} Trainable Parameter Count} \\ \midrule
Encode & GeLU & 256$\times$5 & & \\ 
Decode & GeLU & 3$\times$256$\times$5 & \multirow{-2}{*}{sum} & \multirow{-2}{*}{1262083} \\ \botrule
\end{tabular}
\end{table}

==> tables/Tab.2.tex <==
\begin{table}[!htbp]
\centering
\caption{Range of Variables }\label{tab:res1DataSet}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Variable} & \textbf{Range} \\\midrule
\(c\) : Control variable & [-1; 5] \\
\(x_0\) : Initial condition $x$ & [5; 50] \\
\(y_0\) : Initial condition $y$ & [5; 15] \\
\(t\) : Time interval  & [0; 30] \\
\botrule
\end{tabular}
\end{table}

==> tables/Tab.3.tex <==
\begin{table}[!htbp]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{Training process summary}\label{tab:trainprocess}
\begin{tabular}{@{}llll@{}}
\toprule
                      & \multicolumn{1}{c|}{\textbf{Set Transformer}} & \textbf{OASIS} \\ \midrule
\textbf{Optimizer}        & \multicolumn{2}{c}{Adam}              \\ \midrule
\textbf{Loss function}           & \multicolumn{2}{c}{$\mathcal{L}_{\Xi} + \lambda_0 \mathcal{L}_{ode} + \lambda_1 \mathcal{L}_{reg} $=$\left \| \Xi -\hat{\Xi} \right \|_2 + \lambda_0\left \| \frac{d\widetilde{X}}{dt} - \Theta(\widetilde{X},C)\hat{\Xi} \right \|_1 + \lambda_1\left \| W \right \|_1$}              \\ \midrule
\textbf{Learning rate}           & \multicolumn{2}{c}{$\left [ 10^{-3},~4\times 10^{-4},~10^{-4},~10^{-5},~10^{-6},~10^{-7},~10^{-8} \right ]$}              \\ \midrule
\textbf{Epochs}           & \multicolumn{2}{c}{[2000,~2000,~4000,~2000,~2000,~2000,~2000]}              \\ \midrule
\textbf{Input Shape}  & \multicolumn{1}{c|}{$\left [Batch size,~time,~features \right ]$ : $\left [Batch size,~10,~4 \right ]$       }      &     $\left [Batch size,~1,~4 \right ]$        \\ \midrule
\textbf{Output Shape} & \multicolumn{2}{c}{$\left [Batch size,~coefficients \right ]$ : $\left [Batch size,~20 \right ]$}                            \\ \botrule
\end{tabular}
\end{table}

==> tables/Tab.4.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set Transformer and OASIS in terms of MAPE error for extrapolation through local dynamics identification with a time window of 10 steps}
\label{RESL_10_}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{10}$ & $x$ & \textbf{0.43} & 1.01 & \textbf{0.76} & 3.75 & \textbf{5.36} & 44.64 \\
 & $y$ & \textbf{0.67} & 1.90 & \textbf{1.07} & 3.27 & \textbf{5.36} & 44.64 \\\midrule
2$\times \Delta t_{10}$ & $x$ & \textbf{1.35} & 2.35 & \textbf{3.63} & 9.73 & \textbf{5.36} & 42.86 \\
 & $y$ & \textbf{3.65} & 6.31 & \textbf{17.01} & 21.60 & \textbf{5.36} & 42.86 \\\midrule
3$\times \Delta t_{10}$ & $x$ & \textbf{1.93} & 3.21 & \textbf{4.21} & 10.28 & \textbf{7.14} & 41.07 \\
 & $y$ & \textbf{3.28} & 6.24 & \textbf{11.06} & 19.00 & \textbf{7.14} & 41.07 \\\midrule
4$\times \Delta t_{10}$ & $x$ & \textbf{4.09} & 5.44 & \textbf{12.20} & 15.40 & \textbf{3.57} & 39.29 \\
 & $y$ & \textbf{5.34} & 8.45 & \textbf{18.76} & 24.83 & \textbf{3.57} & 39.29 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.5.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set Transformer and OASIS in terms of MAPE error for extrapolation through local dynamics identification with a time window of 15 steps}
\label{RESL_15_}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{15}$ & $x$ & 1.00 & \textbf{0.83} & 1.54 & \textbf{1.22} & \textbf{7.14} & 51.79 \\
 & $y$ & \textbf{0.88} & 2.92 & \textbf{1.50} & 4.63 & \textbf{7.14} & 51.79 \\\midrule
2$\times \Delta t_{15}$ & $x$ & \textbf{2.41} & 2.81 & \textbf{3.86} & 5.12 & \textbf{7.14} & 51.79 \\
 & $y$ & \textbf{2.26} & 5.49 & \textbf{2.75} & 8.98 & \textbf{7.14} & 51.79 \\\midrule
3$\times \Delta t_{15}$ & $x$ & \textbf{3.49} & 5.11 & \textbf{5.84} & 11.79 & \textbf{5.36} & 44.64 \\
 & $y$ & \textbf{2.88} & 7.83 & \textbf{5.56} & 19.44 & \textbf{5.36} & 44.64 \\\midrule
4$\times \Delta t_{15}$ & $x$ & \textbf{6.24} & 8.09 & \textbf{14.70} & 22.14 & \textbf{3.57} & 44.64 \\
 & $y$ & \textbf{5.20} & 11.80 & \textbf{16.38} & 38.38 & \textbf{3.57} & 44.64 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.6.tex <==
\begin{table}[h]
\centering\caption{Comparison between the two methods Set Transformer and OASIS in terms of MAPE error for extrapolation through local dynamics identification with a time window of 20 steps}
\label{RESL_20_}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}llrrrrrr}
\toprule%
& &\multicolumn{2}{@{}c@{}}{mean} & \multicolumn{2}{@{}c@{}}{90\%} & \multicolumn{2}{@{}c@{}}{divergence (\%)} \\\cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}%
  &  & SETTR & OASIS & SETTR & OASIS & SETTR & OASIS \\
\midrule


1$\times \Delta t_{20}$ & $x$ & 2.42 & \textbf{1.09} & 3.99 & \textbf{1.84} & \textbf{7.14} & 55.36 \\
 & $y$ & \textbf{1.03} & 3.89 & \textbf{1.78} & 6.15 & \textbf{7.14} & 55.36 \\\midrule
2$\times \Delta t_{20}$ & $x$ & 5.10 & \textbf{4.41} & \textbf{8.79} & 9.15 & \textbf{7.14} & 50.00 \\
 & $y$ & \textbf{2.08} & 7.14 & \textbf{3.79} & 11.86 & \textbf{7.14} & 50.00 \\\midrule
3$\times \Delta t_{20}$ & $x$ & \textbf{9.90} & 10.17 & \textbf{15.92} & 23.57 & \textbf{7.14} & 44.64 \\
 & $y$ & \textbf{6.51} & 14.75 & \textbf{16.66} & 39.65 & \textbf{7.14} & 44.64 \\\midrule
4$\times \Delta t_{20}$ & $x$ & \textbf{9.28} & 10.25 & \textbf{14.16} & 24.59 & \textbf{3.57} & 53.57 \\
 & $y$ & \textbf{4.46} & 8.95 & \textbf{9.60} & 23.78 & \textbf{3.57} & 53.57 \\

\botrule
\end{tabular*}
\end{table}

==> tables/Tab.7.tex <==
\begin{table}[!htbp]
\centering
\caption{Range of Variables}\label{tab:res2DataSet}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Variables} & \textbf{Range} \\
\hline
\(\sigma\) variations & [8; 12] \\

\(\rho\) variations & [20; 35] \\

\(\beta\) variations & [0; 4] \\

\(x_0\) variations & [-5; 5] \\

\(y_0\) variations & [4; 50] \\

\(z_0\) variations & [5; 15] \\

\(t\) train and validation & [0, 10[ \\

\(t\) test & [0, 20[ \\
\botrule
\end{tabular}
\end{table}

==> tables/Tab.8.tex <==
\begin{table}[!htbp]
\centering

\caption{Training process summary}\label{tab:trainprocess2}
\begin{tabular}{@{}lc|c@{}}
\toprule
                      & \multicolumn{1}{c}{\textbf{Deep Set}} & \textbf{Set Transformer} \\ \hline
\textbf{Optimizer}        & \multicolumn{2}{c}{Adam}              \\ \midrule
\textbf{Loss function}           & \multicolumn{2}{c}{$\left \| \widetilde{\Xi} -\hat{\Xi} \right \|_2 + \lambda_0\left \| \frac{d\widetilde{X}}{dt} - \Theta(\widetilde{X},C)\hat{\Xi} \right \|_1$}              \\ \midrule
\textbf{Learning rate}           & \multicolumn{2}{c}{$\left [ 4\times10^{-4},~5\times10^{-5},~10^{-5},~5\times10^{-6},~10^{-6} \right ]$}              \\ \midrule
\textbf{Epochs}           & \multicolumn{2}{c}{[400,~400,~400,~400,~400]}              \\ \midrule
\textbf{Input Shape}  & \multicolumn{2}{c}{$\left [Batchsize,~time,~Features \right ] = [Batchsize,~variable,~4]$}         \\ \midrule
\textbf{Output Shape} & \multicolumn{2}{c}{$\left [Batchsize,~3 \right ]$}                            \\ \botrule
\end{tabular}
\end{table}

==> tables/Tab.9.tex <==
\begin{table}[!htbp]
\centering
\caption{Range of characteristics for train, validation and test}\label{tab:rngcharacteristics}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Variables} & \textbf{Range} & \textbf{Distribution}\\
\hline\\
$\alpha_{ref}$  & [$8\times10^{-7};~1.2\times10^{-6}$] & $\mathcal{N}(10^{-6},~~(5\times10^{-8})^2)$\\
$\mathrm{ratio}$  & [$40;~80$] & $\mathcal{N}(60,~~(8)^2)$\\
$\mathrm{G}$  & [$0.001;~0.009$] & Sobol\\
Time $t$  & [$0;~200$] & - \\
\botrule
\end{tabular}
\end{table}
